Gaussian breeding for encoding a qubit in propagating light

Practical quantum computing requires robust encoding of logical qubits in physical systems to protect fragile quantum information. Currently, the lack of scalability limits the logical encoding in most physical systems, and thus the high scalability of propagating light can be a game changer for realizing a practical quantum computer. However, propagating light also has a drawback: the difficulty of logical encoding due to weak nonlinearity. Here, we propose Gaussian breeding that encodes arbitrary Gottesman-Kitaev-Preskill (GKP) qubits in propagating light. The key idea is the efficient and iterable generation of quantum superpositions by photon detectors, which is the most widely used nonlinear element in quantum propagating light. This formulation makes it possible to systematically create the desired qubits with minimal resources. Our simulations show that GKP qubits above a fault-tolerant threshold, including ``magic states'', can be generated with a high success probability and with a high fidelity exceeding 0.99. This result fills an important missing piece toward practical quantum computing.

==> ncctools/source/README <==
README for the `ncctools' bundle
================================

This `bundle' consists of LaTeX2e packages written and supported by
Alexander I. Rozhenko.

The documented source code of all packages is in files with extension
`.dtx'.  To install the bungle, run

  latex ncctools.ins

It will produce the package files from all `.dtx' files.
The files with extensions `.sty' should then be moved to a directory
on LaTeX's standard input path.

License Agreement
=================

This material is subject to the LaTeX Project Public License.
See http://www.ctan.org/tex-archive/help/Catalogue/licenses.lppl.html
for the details of that license.

NOTE (docstrip version)
***********************
****
**** If   latex ncctools.ins
**** produces the `docstrip interactive mode' prompt:
****
****   * First type the extension of your input file(s):  *
****   \infileext=
****
**** Then your version of docstrip is too old.
**** Quit (eg by hitting `enter' to all questions) and get a newer
**** docstrip.tex. It must be at least version 2.4.
****
**** A suitable docstrip.tex may be found from `CTAN' archives such as
**** ftp.dante.de   tex-archive/macros/latex/unpacked/docstrip.tex
****
**** Docstrip is part of the base LaTeX distribution, so if you have
**** an old docstrip then your LaTeX is out of date and you may consider
**** getting the whole of that directory and re-installing LaTeX.
**** However you need to fetch only the file docstrip.tex to unpack
**** this tools distribution with your existing format.


Documentation for the individual documented packages may then be
obtained by running LaTeX on the `.dtx' files.

For example:

  latex manyfoot.dtx

will produce the file manyfoot.dvi, documenting the manyfoot package.

***NOTE****
Copyright is maintained by Alexander I. Rozhenko.

All the packages in this bundle are released under the restrictions
detailed below.

The file manifest.txt contains a list of files in the distribution.


Reporting Bugs
==============

To report a problem or bug in any of these packages, describe it in free
form and send it me to e-mail address

        rozhenko@oapmg.sscc.ru

Type the `NCCTOOLS' word in the subject of letter. This guarantees
that your letter will be not deleted as spam.

When reporting bugs, please produce a small test file that shows the
problem, and ensure that you are using the current version of the
package, and of the base LaTeX software.


Distribution of unchanged versions
==================================

  Redistribution of unchanged files is allowed provided that this
  readme file is included and all the files for a package are
  distributed together.

Generation and distribution of changed versions
===============================================

  The generation of changed versions of the files included in these
  packages is allowed under the restrictions listed in the file
  legal.txt in the base LaTeX distribution.  In particular you should:

  - rename the file before you make any changes to it.

  - change the error report address so that I do not get sent error
    reports for files *not* maintained by me.

  The distribution of changed versions of the files included in these
  packages is allowed under the restrictions listed in the file
  legal.txt in the base LaTeX distribution.  In particular you should:

  - also distribute the unmodified version of the file.

